Stop Looking for Important Tokens in Multimodal Language Models: Duplication Matters More

Vision tokens in multimodal large language models often dominate huge computational overhead due to their excessive length compared to linguistic modality. Abundant recent methods aim to solve this problem with token pruning, which first defines an importance criterion for tokens and then prunes the unimportant vision tokens during inference. However, in this paper, we show that the importance is not an ideal indicator to decide whether a token should be pruned. Surprisingly, it usually results in inferior performance than random token pruning and leading to incompatibility to efficient attention computation operators.Instead, we propose DART (Duplication-Aware Reduction of Tokens), which prunes tokens based on its duplication with other tokens, leading to significant and training-free acceleration. Concretely, DART selects a small subset of pivot tokens and then retains the tokens with low duplication to the pivots, ensuring minimal information loss during token pruning. Experiments demonstrate that DART can prune 88.9% vision tokens while maintaining comparable performance, leading to a 1.99$\times$ and 2.99$\times$ speed-up in total time and prefilling stage, respectively, with good compatibility to efficient attention operators. Our codes are available at https://github.com/ZichenWen1/DART.

==> latex/content/Methodology.tex <==
\section{Methodology}
\subsection{Preliminary}
\label{sec:preliminary}
\mypara{Architecture of MLLM.}
% The MLLM architectures generally consist of three components: a visual encoder, a modality projector, and a LLM. The visual encoder, typically a pre-trained image encoder like CLIP's vision model, converts input images into visual tokens. The projector module aligns these visual tokens with the LLM's word embedding space, enabling the LLM to process visual data effectively. The LLM then integrates the aligned visual and textual information to generate responses.
The architecture of Multimodal Large Language Models (MLLMs) typically comprises three core components: a visual encoder, a modality projector, and a language model (LLM). Given an image $I$, the visual encoder and a subsequent learnable MLP are used to encode $I$ into a set of visual tokens $e_v$. These visual tokens $e_v$ are then concatenated with text tokens $e_t$ encoded from text prompt $p_t$, forming the input for the LLM. The LLM decodes the output tokens $y$ sequentially, which can be formulated as:
\begin{equation}
\label{eq1}
    y_i = f(I, p_t, y_0, y_1, \cdots, y_{i-1}).
\end{equation}

\mypara{Computational Complexity.}  
To evaluate the computational complexity of MLLMs, it is essential to analyze their core components, including the self-attention mechanism and the feed-forward network (FFN). The total floating-point operations (FLOPs) required can be expressed as:  
\begin{equation}
\text{Total FLOPs} = T \times (4nd^2 + 2n^2d + 2ndm),
\end{equation}  
where $T$ denotes the number of transformer layers, $n$ is the sequence length, $d$ represents the hidden dimension size, and $m$ is the intermediate size of the FFN.  
This equation highlights the significant impact of sequence length $n$ on computational complexity. In typical MLLM tasks, the sequence length is defined as: 
\begin{equation}
    n = n_S + n_I + n_Q, 
\end{equation}
where $n_I$, the tokenized image representation, often dominates, sometimes exceeding other components by an order of magnitude or more.  
As a result, minimizing $n_I$ becomes a critical strategy for enhancing the efficiency of MLLMs.

\subsection{Beyond Token Importance: Questioning the Status Quo}
Given the computational burden associated with the length of visual tokens in MLLMs, numerous studies have embraced a paradigm that utilizes attention scores to evaluate the significance of visual tokens, thereby facilitating token reduction.
Specifically, in transformer-based MLLMs, each layer performs attention computation as illustrated below:
\begin{equation}
   \text{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}\left(\frac{\mathbf{Q} \cdot \mathbf{K}^\mathbf{T}}{\sqrt{d_k}}\right)\cdot \mathbf{V},
\end{equation}
where $d_k$ is the dimension of $\mathbf{K}$. The result of $\text{Softmax}(\mathbf{Q}\cdot \mathbf{K}^\mathbf{T}/\sqrt{d_k})$ is a square matrix known as the attention map.
Existing methods extract the corresponding attention maps from one or multiple layers and compute the average attention score for each visual token based on these attention maps:
\begin{equation}
    \phi_{\text{attn}}(x_i) = \frac{1}{N} \sum_{j=1}^{N} \text{Attention}(x_i, x_j),
\end{equation}
where $\text{Attention}(x_i, x_j)$ denotes the attention score between token $x_i$ and token $x_j$, $\phi_{\text{attn}}(x_i)$ is regarded as the importance score of the token $x_i$, $N$ represents the number of visual tokens.
Finally, based on the importance score of each token and the predefined reduction ratio, the most significant tokens are selectively retained:
\begin{equation}
    \mathcal{R} = \{ x_i \mid (\phi_{\text{attn}}(x_i) \geq \tau) \},
\end{equation}
where $\mathcal{R}$ represents the set of retained tokens, and $\tau$ is a threshold determined by the predefined reduction ratio.

\noindent{\textbf{Problems:}} Although this paradigm has demonstrated initial success in enhancing the efficiency of MLLMs, it is accompanied by several inherent limitations that are challenging to overcome.

First, when it comes to leveraging attention scores to derive token importance, it inherently lacks full compatibility with Flash Attention, resulting in limited hardware acceleration affinity and diminished acceleration benefits.

Second, does the paradigm of using attention scores to evaluate token importance truly ensure the effective retention of crucial visual tokens? Our empirical investigations reveal that it is not the optimal approach.

% As illustrated in Figure~\ref{fig:random_vs_others}, performance evaluations on certain benchmarks show that methods meticulously designed based on this paradigm sometimes underperform compared to randomly retaining the same number of visual tokens.
Performance evaluations on certain benchmarks, as illustrated in Figure~\ref{fig:random_vs_others}, demonstrate that methods meticulously designed based on this paradigm sometimes underperform compared to randomly retaining the same number of visual tokens.

% As depicted in Figure~\ref{fig:teaser_curry}, which visualizes the results of token reduction, the selection of visual tokens based on attention scores exhibits a noticeable bias, favoring tokens located in the lower-right region of the image—those positioned later in the visual token sequence. However, it is evident that the lower-right region is not always the most significant in every image.
% Furthermore, in Figure~\ref{fig:teaser_curry}, we present the outputs of the original LLaVA-1.5-7B, FastV, and our proposed \algname. Notably, FastV introduces more hallucinations compared to the vanilla model, while \algname demonstrates a noticeable trend of reducing hallucinations.
% We suppose that this phenomenon arises because the important-based method, which relies on attention scores, tends to retain visual tokens that are concentrated in specific regions of the image due to the inherent bias in attention scores. As a result, relying on only a portion of the image often leads to outputs that are inconsistent with the overall image content. In contrast, \algname primarily removes highly duplication tokens and retains tokens that are more evenly distributed across the entire image, enabling it to make more accurate and consistent judgments.
%--------------- shorter version ---------------------
Figure~\ref{fig:teaser_curry} visualizes the results of token reduction, revealing that selecting visual tokens based on attention scores introduces a noticeable bias toward tokens in the lower-right region of the image—those appearing later in the visual token sequence. However, this region is not always the most significant in every image. Additionally, we present the outputs of the original LLaVA-1.5-7B, FastV, and our proposed \algname. Notably, FastV generates more hallucinations compared to the vanilla model, while \algname effectively reduces them. 
We attribute this to the inherent bias of attention-based methods, which tend to retain tokens concentrated in specific regions, often neglecting the broader context of the image. In contrast, \algname removes highly duplication tokens and preserves a more balanced distribution across the image, enabling more accurate and consistent outputs.

\subsection{Token Duplication: Rethinking Reduction}
Given the numerous drawbacks associated with the paradigm of using attention scores to evaluate token importance for token reduction, \textit{what additional factors should we consider beyond token importance in the process of token reduction?}
Inspired by the intuitive ideas mentioned in \secref{sec:introduction} and the phenomenon of tokens in transformers tending toward uniformity (i.e., over-smoothing)~\citep{nguyen2023mitigating, gong2021vision}, we propose that token duplication should be a critical focus.

Due to the prohibitively high computational cost of directly measuring duplication among all tokens, we adopt a paradigm that involves selecting a minimal number of pivot tokens. 
\begin{equation}
    \mathcal{P} = \{p_1, p_2, \dots, p_k\}, \quad k \ll n,
\end{equation}
where $p_i$ denotes pivot token, $\mathcal{P}$ represents the set of pivot tokens and $n$ means the length of tokens.

Subsequently, we compute the cosine similarity between these pivot tokens and the remaining visual tokens:
\begin{equation}
    dup (p_i, x_j) = \frac{p_i \cdot x_j}{\|p_i\| \cdot \|x_j\|}, \quad p_i \in \mathcal{P}, \, x_j \in \mathcal{X},
\end{equation}
where $dup (p_i, x_j)$ represents the token duplication score between $i$-th pivot token $p_i$ and $j$-th visual token $x_j$,
ultimately retaining those tokens that exhibit the lowest duplication with the pivot tokens.
\begin{equation}
    \mathcal{R} = \{ x_j \mid \min_{p_i \in \mathcal{P}} dup (p_i, x_j) \leq \epsilon \}.
\end{equation}
Here, $\mathcal{R}$ denotes the set of retained tokens, and $\epsilon$ is a threshold determined by the reduction ratio.

Our method is orthogonal to the paradigm of using attention scores to measure token importance, meaning it is compatible with existing approaches. Specifically, we can leverage attention scores to select pivot tokens, and subsequently incorporate token duplication into the process.

However, this approach still does not fully achieve compatibility with Flash Attention. To this end, we explored alternative strategies for selecting pivot tokens, such as using K-norm, V-norm\footnote{Here, the K-norm and V-norm refer to the L1-norm of K matrix and V matrix in attention computing, respectively.}, or even random selection. Surprisingly, we found that all these methods achieve competitive performance across multiple benchmarks. This indicates that our token reduction paradigm based on token duplication is not highly sensitive to the choice of pivot tokens. Furthermore, it suggests that removing duplicate tokens may be more critical than identifying ``important tokens'', highlighting token duplication as a potentially more significant factor to consider in token reduction.
The selection of pivot tokens is discussed in greater detail in \secref{pivot_token_selection}.
% 加个总结


==> latex/content/introduction_backup.tex <==
\section{Introduction}\label{sec:introduction}
% 引入mllm
\input{latex/figure/teaser_curry}
The advent of large language models (LLMs)~\citep{radford2019language, brown2020language, achiam2023gpt, touvron2023llama, peng2023instruction, bi2024deepseek} and pre-trained vision models~\citep{radford2021learning, liu2025grounding} has propelled multimodal large language  models (MLLMs)~\citep{team2023gemini, Qwen-VL, wang2024qwen2, chen2023internvl, li2024mini, li2023blip} by advancing connections between visual and linguistic modalities through linear projection~\citep{li2024llava} or q-former~\citep{instructblip}. 
% With modal alignment and visual instruction fine-tuning \citep{du2021glm, liu2023improvedllava, zhu2023minigpt}, recent MLLMs successfully adapt LLMs to the vision domain and inherit their perception and reasoning abilities.
These MLLMs exhibit remarkable capabilities across a diverse range of multimodal tasks, including image captioning, visual question answering (VQA), video understanding~\citep{wang2024internvideo2}, and multimodal reasoning~\citep{wang2024exploring}. % todo: add reference
\input{latex/figure/random_vs_others.tex}

% 指出现有mllm中image tokens占比过高且信息稀疏
% 尽管各种mllm展现出了promising performance，但与文本模态相比过长的vision token给mllm带来了巨大存储和计算量过大的挑战，尤其是当处理超高分辨率图像，视频理解以及多图场景。
Although various MLLMs have demonstrated promising performance, the significantly longer vision tokens compared to the linguistic modality pose substantial challenges in terms of massive storage and computational overhead~\citep{ju2023turbo}, especially when handling high-resolution images~\citep{li2024mini} and multi-frame video~\citep{tang2023video}.
For instance, processing a single video with Video-LLaVA~\citep{lin2023video} involves extracting $8$ frames, generating $2048$ vision tokens—significantly surpassing the number of text tokens.

This limits the application scenarios of MLLMs, especially in cases that require low latency, such as autonomous driving~\citep{jia2023adriver} and real-time interactions~\citep{fu2024vita}.

% 介绍现有的解决mllm中image token过长的方法
% 一些方法需要更改组件然后训练

% 1. fastv->无法兼容fa
% 2. sparsevlm->无法兼容fa
% 3. mustdrop->无法兼容fa

Despite occupying a significant portion of the input sequence, vision tokens lack the information density like text modality~\citep{marr2010vision}.
To address this issue, several studies have sought to extract more compact image representations by enhancing the image encoder or projector~\citep{alayrac2022flamingo, li2023llama, instructblip, cha2024honeybee}.
However, these methods typically necessitate substantial modifications to the MLLM architecture and demand extensive training.
% 与此同时，一些最近的工作尝试用training-free的方法减少vision tokens。
While some recent works have explored training-free approaches to reduce vision tokens by token pruning, which firstly defines the importance score of each token, and then prunes the most unimportant tokens during the inference phrase~\citep{chen2024image, zhang2024sparsevlm, liu2024multi}. 
These importance-based token pruning methods implicitly assumes that there exists a static and oracle score that can characterize the influence of this token on model prediction. However, in this paper, we argue that this ``importance'' perspective exist several serious problems as follows.

\textbf{``Importance'' scores ignore the interaction between different tokens during pruning. For two similar tokens, }

% 独立性假设
% 效果不好
% 不支持flashattention
% 位置bias



%the influence of pruning a token can be considered independently with other tokens. Obviously, this assumption ignores the interaction between multiple tokens. In other words, the choice of pruning a token should not only judged by itself, but also influenced by the pruning choice of other tokens, especially influenced by the tokens which are similar to this token.



Due to their reliance on attention scores for assessing the importance of vision tokens, these methods struggle to integrate smoothly with Flash Attention~\citep{dao2022flashattention, dao2023flashattention2}, significantly limiting their acceleration benefits.
% Additionally, these approaches place excessive emphasis on the importance of tokens, overlooking the crucial role that token duplication plays in token reduction.

% our method
% 在这篇工作中，我们试图回答三个问题：
% 1. 能否不利用attention score挑选tokens,做到兼容flash attention？
% 2. 通过衡量token重要性进行token reduction是最优的？
% 3. 除了token重要性，在token reduction中还需要关注什么？
% 加一句:为了解决这一问题，我们尝试设计能够与flash attention兼容的token reduction方法。
To address this issue, we aim to develop token reduction methods that are compatible with flash attention.
Before that, we delve into two intriguing research questions:
\textbf{Q1:} \textit{Is it optimal for the attention score to measure token importance to guide the token reduction paradigm?}
\textbf{Q2:} \textit{Beyond token importance, what factors should be considered in token reduction?}
 \\
\textbf{Is it optimal for the attention score to measure token importance to guide the token reduction paradigm?}
 % TODO: refine this sentence.
We conducted a comparative analysis of token reduction performance across random token selection, FastV~\citep{chen2024image}, and SparseVLM~\citep{zhang2024sparsevlm}. As illustrated in Figure~\ref{fig:random_vs_others}, random token selection even outperforms both FastV and SparseVLM on certain benchmarks. This suggests that relying on attention scores to measure token importance for reduction may not be optimal. Instead, it is crucial to explore factors beyond token importance to address the inherent limitations of attention scores in flash attention.
% 加个柱状图来说明random token selection有时候好于依据attent score精心设计的fastv & sparsevlm
% 根据图讲解下，得到结论：在token reduction中考虑token importance不是最优方案。
\\
\textbf{Beyond token importance, what factors should be considered in token reduction?}
% fastv是典型的利用attention score衡量token重要性进行token reduction的方法->画图
 %1. 首先在同一张图像上将fastv保留image token对应的patch可视化出来 vs 我们利用k-norm + token重复性考虑的patch 可视化
 %2. 然后在特征空间进行tsne可视化的对比，展示出我们保留的特征没有太聚集，比较分散
% 顺势引出考虑token重复性在token reduction中的必要性。
Previous research has extensively investigated the over-smoothing phenomenon in transformers~\citep{ nguyen2023mitigating, wang2022anti}, with studies demonstrating that self-attention mechanism inherently drives token representations toward increasingly identical latent states~\citep{gong2021vision, wang2023label}.
This insight inspires us to incorporate token duplication into the token reduction. When multiple tokens exhibit identical or highly similar representations, it is natural to retain only one of them for prediction, thereby maintaining efficiency without compromising performance.
% \input{latex/figure/radar_compare.tex}
\input{latex/figure/latency_vs_performance}

In this work, building upon the insights from the aforementioned discussions, we propose a plug-and-play token reduction method grounded in token duplication without training, which is designed to be fully compatible with flash attention. 
% Specifically, during the forward inference process of the MLLMs, at the shallow layers, we first select a small subset of pivot tokens (no more than 2\% of the total tokens) based on their high $\mathrm{K}_{\mathrm{norm}}$ values. We then compute the cosine similarity between these selected tokens and the remaining image tokens. Based on the predefined reduction ratio, we retain the image tokens with the lowest cosine similarity, as we hypothesize that image tokens exhibiting high feature redundancy with the selected tokens contribute minimally to subsequent predictions.
% Specifically, during the inference process of MLLMs, we begin by selecting a small subset of pivot tokens—comprising no more than $2\%$ of the total tokens—based on their elevated K-norm values in the shallow layers. 
Specifically, during the inference process of MLLMs, we begin by selecting a small subset of pivot tokens, comprising no more than $2\%$ of the total tokens in the shallow layers. 
We then calculate the cosine similarity between pivot tokens and the remaining image tokens. Guided by a predefined reduction ratio, we retain only those image tokens with the lowest cosine similarity. The entire process is highly efficient, completing in no more than $0.08$ seconds. This approach is motivated by the prior insights~\citep{gong2021vision} that image tokens exhibiting high feature duplication with the pivot tokens contribute negligibly to predictions. Moreover, since our entire process operates independently of attention scores, it is fully compatible with flash attention, ensuring seamless integration and enhanced computational efficiency.
In summary, the contributions of this work are three-fold:
\begin{itemize}
    \item \textbf{Rethink Token Important} Through empirical analysis, we demonstrate the suboptimality of relying on attention scores to measure token importance to guide the token reduction paradigm.
    \item \textbf{Token Duplication as a Key Factor} Building on the concept of token duplication, we introduce a training-free, plug-and-play token reduction method that seamlessly integrates with flash attention. 
    \item ...
\end{itemize}



==> latex/content/table/OCRBench_details.tex <==

\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.0}
\scalebox{0.8}{
\begin{tabular}{c|ccccc|c}
\toprule[1.5pt]
\textbf{Method} & \textbf{Recog.} & \textbf{VQA}$^{\text{Scene}}$ & \textbf{VQA}$^{\text{Doc}}$ & \textbf{KIE} & \textbf{HMER} & \textbf{Final Score} \\
\hline

\rowcolor{mygray}
LLaVA-1.5-7B & \multicolumn{6}{c}{\textit{Upper Bound, 576 Tokens} \ $\textbf{(100\%)}$}\\
\textcolor{gray}{Vanilla} & \textcolor{gray}{160} & \textcolor{gray}{117} & \textcolor{gray}{15} & \textcolor{gray}{5} & \textcolor{gray}{0} & \textcolor{gray}{297} \\
\hline
\rowcolor{mygray}
LLaVA-1.5-7B & \multicolumn{6}{c}{\textit{Retain 128 Tokens} \ $\fg{(\downarrow 77.8\%)}$} \\

FastV \texttt{\scriptsize{(ECCV24}} & 160 & 114 & 10 & 1 & 0 & 285 \\
% HiRED \texttt{\scriptsize{(AAAI25)}} & 51 & 110 & \textbf{21} & \textbf{9} & 0 & 191  \\
SparseVLM \texttt{\scriptsize{(2024.10)}} & 156 & 110 & 13 & 1 & 0 & 280 \\
PDrop \texttt{\scriptsize{(2024.10)}} & 162 & 113 & 12 & 0 & 0 & 287    \\
MustDrop \texttt{\scriptsize{(2024.11}} & 156 & 110 & 13 & 2 & 0 & 281  \\
DART (Ours) & \textbf{165} & \textbf{114} & 13 & 4 & \textbf{0} & \textbf{296}  \\





\hline
\hline
\rowcolor{mygray}
LLaVA-Next-7B & \multicolumn{6}{c}{\textit{Upper Bound, 2880 Tokens} \ $\textbf{(100\%)}$}\\
\textcolor{gray}{Vanilla} & \textcolor{gray}{193} & \textcolor{gray}{150} & \textcolor{gray}{76} & \textcolor{gray}{98} & \textcolor{gray}{0} & \textcolor{gray}{517} \\

\hline
\rowcolor{mygray}
LLaVA-Next-7B & \multicolumn{6}{c}{\textit{Retain 320 Tokens} \ $\fg{(\downarrow 88.9\%)}$} \\
FastV \texttt{\scriptsize{(ECCV24)}} & 174 & 133 & 33 & 34 & 0 & 374 \\
% HiRED \texttt{\scriptsize{(AAAI25)}} & 175 & \textbf{151} & \textbf{47} & 30 & \textbf{1} & 404    \\
SparseVLM \texttt{\scriptsize{(2024.10)}} & 130 & 102 & 22 & 16 & 0 & 270 \\
PDrop \texttt{\scriptsize{(2024.10)}} & 109 & 111 & 25 & 14 & 0 & 259 \\
MustDrop \texttt{\scriptsize{(2024.11}} & 181 & 131 & 38 & 32 & 0 & 382 \\
DART (ours) & \textbf{195} & 137 & 39 & \textbf{35} & 0 & \textbf{406} \\




\bottomrule[1.5pt]
\end{tabular}
}
\caption{\textbf{Detailed comparison on OCRBench}, including Text Recognition, Scene Text-centric VQA, Doc-oriented VQA, Key Information Extraction, Handwritten Mathematical Expression Recognition.}
\end{table*}

==> latex/content/table/image_understanding.tex <==
% \renewcommand{\multirowsetup}{\centering}
% \definecolor{mygray}{gray}{.92}
% \definecolor{ForestGreen}{RGB}{34,139,34}
% \newcommand{\fg}[1]{\mathbf{\mathcolor{ForestGreen}{#1}}}
% \definecolor{Forestred}{RGB}{220,50,50}
% \newcommand{\fr}[1]{\mathbf{\mathcolor{Forestred}{#1}}}
% \begin{table*}[t]
%     \centering
%     % \hspace{2mm}
%     \setlength{\tabcolsep}{2.8pt}
%     \renewcommand{\arraystretch}{1.4}
%     \footnotesize
% 	\centering
% 	\caption{\textbf{Performance of SparseLLaVA under different vision token configurations.} The vanilla number of vision tokens is $576$. The first line of each method is the raw accuracy of benchmarks, and the second line is the proportion relative to the upper limit. The last column is the average value.}
%     \vspace{2mm}
% 	\label{tab:main}
%     \begin{tabular}{p{2cm}|c c c c c c c c | c}
%         \toprule[1.5pt]
%         \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{V2}}$ & \textbf{VQA}$^{\text{Text}}$ & \textbf{ConB} &\makecell[c]{\textbf{Avg}.}\\
%         \hline
%         \rowcolor{mygray}
%         \multicolumn{10}{c}{\textit{Upper Bound, 576 Tokens} \ $\textbf{(100\%)}$}\\
%         \multirow{2}*{Vanilla} & 61.9 & 64.7 & 1862 & 85.9 & 69.5 & 78.5 & 58.2 & 19.8 & \multirow{2}*{100\%} \\
%         ~ & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & ~ \\
%         \hline

%         \rowcolor{mygray}
%         \multicolumn{10}{c}{\textit{Retain 192 Tokens} \ $\fg{(\downarrow 66.7\%)}$} \\
%         \multirow{2}*{ToMe \texttt{\scriptsize{(ICLR23)}}} & 54.3 & 60.5 & 1563 & 72.4 & 65.2 & 68.0 & 52.1 & 17.4 & \multirow{2}*{88.4\%} \\
%         ~ & 87.7\% & 93.5\% & 83.9\% & 84.3\% & 93.8\% & 86.6\% & 89.5\% & 87.9\% & ~ \\
%         \hline
%         \multirow{2}*{FastV \texttt{\scriptsize{(ECCV24)}}} & 52.7 & 61.2 & 1612 & 64.8 & 67.3 & 67.1 & 52.5 & 18.0 & \multirow{2}*{88.1\%} \\
%         ~ & 85.1\% & 94.6\% & 86.6\% & 75.4\% & 96.8\% & 85.5\% & 90.2\% & 90.9\% & ~ \\
%         \hline
%         \multirow{2}*{SparseVLM} & 57.6 & 62.5 & 1721 & 83.6 & 69.1 & 75.6 & 56.1 & 18.8 & \textbf{95.8\%} \\
%         ~ & 93.1\% & 96.6\% & 92.4\% & 97.3\% & 99.4\% & 96.3\% & 96.4\% & 94.9\% &  $\fr{\uparrow(7.4\%)}$\\
%         \hline

%         \rowcolor{mygray}
%         \multicolumn{10}{c}{\textit{Retain 128 Tokens} \ $\fg{(\downarrow 77.8\%)}$}\\
%         \multirow{2}*{ToMe \texttt{\scriptsize{(ICLR23)}}} & 52.4 & 53.3 & 1343 & 62.8 & 59.6 & 63.0 & 49.1 & 16.0 & \multirow{2}*{80.4\%} \\
%         ~ & 84.7\% & 82.4\% & 72.1\% & 73.1\% & 85.8\% & 80.2\% & 84.4\% & 80.8\% & ~ \\
%         \hline
%         \multirow{2}*{FastV \texttt{\scriptsize{(ECCV24)}}} & 49.6 & 56.1 & 1490 & 59.6 & 60.2 & 61.8 & 50.6 & 17.1 & \multirow{2}*{81.9\%}\\
%         ~ & 80.1\% & 86.7\% & 80.0\% & 69.4\% & 86.6\% & 78.7\% & 86.9\% & 86.4\% & ~\\
%         \hline
%         \multirow{2}*{SparseVLM} & 56.0 & 60.0 & 1696 & 80.5 & 67.1 & 73.8 & 54.9 & 18.5 & \textbf{93.3\%}\\
%         ~ & 90.5\% & 92.7\% & 91.1\% & 93.7\% & 96.5\% & 94.0\% & 94.3\% & 93.4\% & $\fr{\uparrow(11.4\%)}$\\
%         \hline

%         \rowcolor{mygray}
%         \multicolumn{10}{c}{\textit{Retain 64 Tokens} \ $\fg{(\downarrow 88.9\%)}$}\\
%         \multirow{2}*{ToMe \texttt{\scriptsize{(ICLR23)}}} & 48.6 & 43.7 & 1138 & 52.5 & 50.0 & 57.1 & 45.3 & 14.0 & \multirow{2}*{70.2\%}\\
%         ~ & 78.5\% & 67.5\% & 61.1\% & 61.1\% & 71.9\% & 72.7\% & 77.8\% & 70.7\% & ~\\
%         \hline
%         \multirow{2}*{FastV \texttt{\scriptsize{(ECCV24)}}} & 46.1 & 48.0 & 1256 & 48.0 & 51.1 & 55.0 & 47.8 & 15.6 & \multirow{2}*{72.1\%}\\
%         ~ & 74.5\% & 74.2\% & 67.5\% & 55.9\% & 73.5\% & 70.1\% & 82.1\% & 78.8\% & ~\\
%         \hline
%         \multirow{2}*{SparseVLM} & 52.7 & 56.2 & 1505 & 75.1 & 62.2 & 68.2 & 51.8 & 17.7 & \textbf{86.9\%} \\
%         ~ & 85.1\% & 86.9\% & 80.8\% & 87.4\% & 89.4\% & 86.9\% & 89.0\% & 89.4\% & $\fr{\uparrow(14.8\%)}$\\

%         \bottomrule[1.5pt]
% 	\end{tabular}
%      \vspace{-2mm}
% \end{table*}



\renewcommand{\multirowsetup}{\centering}
\definecolor{mygray}{gray}{.92}
\definecolor{ForestGreen}{RGB}{34,139,34}
\definecolor{Forestred}{RGB}{220,50,50}
\begin{table*}[!ht]
    \centering
    \vspace{-1mm}
    % \hspace{2mm}
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{0.9}
    \footnotesize
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c | c c c c c c c c c c| >{\centering\arraybackslash}p{1.0cm}}
        \toprule[1.5pt]
        \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{V2}}$ & \textbf{VQA}$^{\text{Text}}$ & \textbf{VizWiz} & \textbf{OCRBench} & \makecell[c]{\textbf{Avg}.}\\
        \hline
        \rowcolor{mygray}
        LLaVA-1.5-7B & \multicolumn{11}{c}{\textit{Upper Bound, 576 Tokens} \ $\textbf{(100\%)}$}\\
        \textcolor{gray}{Vanilla} & \textcolor{gray}{61.9} & \textcolor{gray}{64.7} & \textcolor{gray}{58.1} & \textcolor{gray}{1862} & \textcolor{gray}{85.9} & \textcolor{gray}{69.5} & \textcolor{gray}{78.5} & \textcolor{gray}{58.2} & \textcolor{gray}{50.0} & \textcolor{gray}{297} & \multirow{1}*{\textcolor{gray}{100\%}} \\
        \hline

        \rowcolor{mygray}
        LLaVA-1.5-7B & \multicolumn{11}{c}{\textit{Retain 192 Tokens} \ $\fg{(\downarrow 66.7\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 54.3 & 60.5 & - & 1563 & 72.4 & 65.2 & 68.0 & 52.1 & - & - & - \\
        FastV \texttt{\scriptsize{(ECCV24)}} & 52.7 & 61.2 & 57.0 & 1612 & 64.8 & 67.3 & 67.1 & 52.5 & 50.8 & 291 & \multirow{1}*{91.2\%} \\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 58.7 & 62.8 & 54.7 & 1737 & 82.8 & 68.4 & 74.9 & 47.4 & 50.1 & 190 & 91.5\%     \\
        FitPrune \texttt{\scriptsize{(AAAI25)}} & \textbf{60.4 }& 63.3 & 56.4 & 1831 & 83.4 & 67.8 & - & 57.4 & 50.9 & - & - \\
        LLaVA-PruMerge \texttt{\scriptsize{(2024.05)}} & 54.3 & 59.6 & 52.9 & 1632 & 71.3 & 67.9 & 70.6 & 54.3 & 50.1 & 253 & 90.8\% \\
        \multirow{1}*{SparseVLM \texttt{\scriptsize{(ICML25)}}} & 57.6 & 62.5 & 53.7 & 1721 & \textbf{83.6} & 69.1 & 75.6 & 56.1 & 50.5 & 292 & 96.3\% \\
        PDrop \texttt{\scriptsize{(2024.10)}} & 57.1 & 63.2 & 56.8 & 1766 & 82.3 & 68.8 & 75.1 & 56.1 & 51.1 & 290 & 96.7\% \\
        FiCoCo-V \texttt{\scriptsize{(2024.11)}} & 58.5 & 62.3 & 55.3 & 1732 & 82.5 & 67.8 & 74.4 & 55.7 & 51.0 & - & 96.1\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 58.2 & 62.3 & 55.8 & 1787 & 82.6 & 69.2 & 76.0 & 56.5 & \textbf{51.4} & 289 & 97.2\% \\
        \algname (Ours) & 60.0 & \textbf{63.6} & \textbf{57.0} & \textbf{1856} & 82.8 & \textbf{69.8} & \textbf{76.7} & \textbf{57.4} & 51.2 & \textbf{296} & \textbf{98.8\%} \\
        \rowcolor{cyan!7}
        \algname$^\dagger$ (Ours) & 60.9 & 66.3 & 59.5 & 1829 & 85.3 & 70.1 & - & 56.8 & 51.3 & 304 & - \\
        \hline

        \rowcolor{mygray}
        LLaVA-1.5-7B & \multicolumn{11}{c}{\textit{Retain 128 Tokens} \ $\fg{(\downarrow 77.8\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 52.4 & 53.3 & - & 1343 & 62.8 & 59.6 & 63.0 & 49.1 & - & - & - \\
        FastV \texttt{\scriptsize{(ECCV24)}} & 49.6 & 56.1 & 56.4 & 1490 & 59.6 & 60.2 & 61.8 & 50.6 & 51.3 & 285 & \multirow{1}*{86.4\%}\\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 57.2 & 61.5 & 53.6 & 1710 & 79.8 & 68.1 & 73.4 & 46.1 & 51.3 & 191 & 90.2\% \\
        FitPrune \texttt{\scriptsize{(AAAI25)}} & 58.5 & 62.7 & 56.2 & 1776 & 77.9 & 68.0 & - & 55.7 & 51.7 & - & - \\
        LLaVA-PruMerge \texttt{\scriptsize{(2024.05)}} & 53.3 & 58.1 & 51.7 & 1554 & 67.2 & 67.1 & 68.8 & 54.3 & 50.3 & 248 & 88.8\%  \\
        SparseVLM
         \texttt{\scriptsize{(ICML25)}} & 56.0 & 60.0 & 51.1 & 1696 & 80.5 & 67.1 & 73.8 & 54.9 & 51.4 & 280 & 93.8\% \\
        PDrop \texttt{\scriptsize{(2024.10)}} & 56.0 & 61.1 & 56.6 & 1644 & \textbf{82.3} & 68.3 & 72.9 & 55.1 & 51.0 & 287 & 95.1\% \\
        FiCoCo-V \texttt{\scriptsize{(2024.11)}} & 57.6 & 61.1 & 54.3 & 1711 & 82.2 & 68.3 & 73.1 & 55.6 & 49.4 & - & 94.9\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 56.9 & 61.1 & 55.2 & 1745 & 78.7 & 68.5 & 74.6 & 56.3 & \textbf{52.1} & 281 & 95.6\% \\
        \algname (Ours) & \textbf{58.7} & \textbf{63.2} & \textbf{57.5} & \textbf{1840} & 80.1 & \textbf{69.1} & \textbf{75.9} & \textbf{56.4} & 51.7 & \textbf{296} & \textbf{98.0\%} \\
        \rowcolor{cyan!7}
        \algname$^\dagger$ (Ours) & 59.8 & 65.6 & 58.3 & 1849 & 84.4 & 70.7 & - & 56.4 & 52.6 & 299 \\
        \hline

        \rowcolor{mygray}
        LLaVA-1.5-7B & \multicolumn{11}{c}{\textit{Retain 64 Tokens} \ $\fg{(\downarrow 88.9\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 48.6 & 43.7 & - & 1138 & 52.5 & 50.0 & 57.1 & 45.3 & - & - & - \\
        FastV \texttt{\scriptsize{(ECCV24)}} & 46.1 & 48.0 & 52.7 & 1256 & 48.0 & 51.1 & 55.0 & 47.8 & 50.8 & 245 & 77.3\% \\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 54.6 & 60.2 & 51.4 & 1599 & 73.6 & 68.2 & 69.7 & 44.2 & 50.2 & 191 & 87.0\% \\
        FitPrune \texttt{\scriptsize{(AAAI25)}} & 52.3 & 58.5 & 49.7 & 1556 & 60.9 & 68.0 & - & 51.2 & 51.1 & - & - \\
        LLaVA-PruMerge \texttt{\scriptsize{(2024.05)}} & 51.9 & 55.3 & 49.1 & 1549 & 65.3 & 68.1 & 67.4 & 54.0 & 50.1 & 250 & 87.4\% \\
        SparseVLM \texttt{\scriptsize{(ICML25)}} & 52.7 & 56.2 & 46.1 & 1505 & 75.1 & 62.2 & 68.2 & 51.8 & 50.1 & 180 & 84.6\% \\
        PDrop \texttt{\scriptsize{(2024.10)}} & 41.9 & 33.3 & 50.5 & 1092 & 55.9 & 68.6 & 69.2 & 45.9 & 50.7 & 250 & 78.1\% \\
        FiCoCo-V \texttt{\scriptsize{(2024.11)}} & 52.4 & 60.3 & 53.0 & 1591 & \textbf{76.0} & 68.1 & 71.3 & 53.6 & 49.8 & - & 91.5\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 53.1 & 60.0 & 53.1 & 1612 & 68.0 & 63.4 & 69.3 & 54.2 & 51.2 & 267 & 90.1\%    \\
        \algname (Ours) & \textbf{55.9} & \textbf{60.6} & \textbf{53.2} & \textbf{1765} & 73.9 & \textbf{69.8} & \textbf{72.4} & \textbf{54.4} & \textbf{51.6} & \textbf{270} & \textbf{93.7\%} \\
        \rowcolor{cyan!7}
        \algname$^\dagger$ (Ours) & 57.1 & 64.7 & 56.7 & 1823 & 79.3 & 71.1 & - & 54.7 & 52.1 & 286 & - \\

        \hline
        \hline
        \rowcolor{mygray}
        LLaVA-Next-7B & \multicolumn{11}{c}{\textit{Upper Bound, 2880  Tokens} \ $\textbf{(100\%)}$}\\
         \textcolor{gray}{Vanilla} & \textcolor{gray}{64.2} & \textcolor{gray}{67.4} & \textcolor{gray}{60.6} & \textcolor{gray}{1851} & \textcolor{gray}{86.5} & \textcolor{gray}{70.1} & \textcolor{gray}{81.8} & \textcolor{gray}{64.9} & \textcolor{gray}{57.6} & \textcolor{gray}{517} &  \textcolor{gray}{100\%} \\
          \hline
       \rowcolor{mygray}
        LLaVA-Next-7B & \multicolumn{11}{c}{\textit{Retain 320 Tokens} \ $\fg{(\downarrow 88.9\%)}$} \\

        FastV \texttt{\scriptsize{(ECCV24)}} & 55.9 & 61.6 & 51.9 & 1661 & 71.7 & 62.8 & 71.9 & 55.7 & 53.1 & 374 & 86.4\% \\
        
        HiRED \texttt{\scriptsize{(AAAI25)}} & 59.3 & 64.2 & 55.9 & 1690 & 83.3 & 66.7 & 75.7 & 58.8 & 54.2 & 404 & 91.8\% \\
        
        LLaVA-PruMerge \texttt{\scriptsize{(2024.05)}} & 53.6 & 61.3 & 55.3 & 1534 & 60.8 & 66.4 & 69.7 & 50.6 & 54.0 & 146 & 79.9\% \\

       SparseVLM \texttt{\scriptsize{(ICML25)}} & 56.1 & 60.6 & 54.5 & 1533 & 82.4 & 66.1 & 71.5 & 58.4 & 52.0 & 270 & 85.9\%  \\

       PDrop \texttt{\scriptsize{(2024.10)}} & 56.4 & 63.4 & 56.2 & 1663 & 77.6 & 67.5 & 73.5 & 54.4 & 54.1 & 259 & 86.8\% \\

        MustDrop \texttt{\scriptsize{(2024.11)}} & 57.3 & 62.8 & 55.1 & 1641 & 82.1 & 68.0 & 73.7 & \textbf{59.9} & 54.0 & 382 & 90.4\%    \\

       FasterVLM \texttt{\scriptsize{(2024.12)}} & 56.9 & 61.6 & 53.5 & 1701 & 83.6 & 66.5 & 74.0 & 56.5 & 52.6 & 401 & 89.8\% \\
       
       GlobalCom$^2$ \texttt{\scriptsize{(2025.01)}} & 57.1 & 61.8 & 53.4 & 1698 & 83.8 & 67.4 & 76.7 & 57.2 & 54.6 & 375 & 90.3\%  \\

       \algname (Ours)& \textbf{61.7} & \textbf{65.3} & \textbf{58.2} & \textbf{1710} & \textbf{84.1} & \textbf{68.4} & \textbf{79.1} & 58.7 & \textbf{56.1} & \textbf{406} & \textbf{93.9\%}  \\

        \bottomrule[1.5pt]
	\end{tabular}}
        \vspace{-2mm}
	\caption{Comparative experiments on image understanding. In all experiments for \algname, tokens are pruned after the second layer with $8$ pivot tokens. The pivot tokens are selected based on the maximum K-norm.}
    \label{tab:main}
     \vspace{-2mm}
\end{table*}



==> latex/content/table/image_understanding_minicpm.tex <==
\renewcommand{\multirowsetup}{\centering}
\definecolor{mygray}{gray}{.92}
\definecolor{ForestGreen}{RGB}{34,139,34}
\definecolor{Forestred}{RGB}{220,50,50}
% \begin{table*}[t]
%     \centering
%     % \hspace{2mm}
%     \scalebox{1.0}{
%     \setlength{\tabcolsep}{3.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \footnotesize
% 	\label{tab:minicpm}
%     \begin{tabular}{@{}lc | c c c c c c c | c}
%         \toprule[1.5pt]
%         \textbf{Method} & Retention Ratio & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} &  \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.}\\
%         \hline

%         MiniCPM-V-2.6 & $\fg{\downarrow 0.00\%}$ & \textcolor{gray}{51.5} & \textcolor{gray}{79.7} & \textcolor{gray}{77.9} & \textcolor{gray}{2267} & \textcolor{gray}{83.2} & \textcolor{gray}{95.6} & \textcolor{gray}{78.5} & \multirow{1}*{\textcolor{gray}{100\%}} \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 66.7\%}$ & 47.8 & 76.5 & 74.8 & 1951 & 77.4 & 91.8 & 70.9 & 92.9\% \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 77.8\%}$ & 47.8 & 73.8 & 71.4 & 1821 & 71.6 & 88.9 & 65.7 & 88.6\% \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 88.9\%}$ & 42.5 & 66.2 & 64.0 & 1405 & 58.0 & 83.5 & 51.9 & 76.1\% \\

%         \bottomrule[1.5pt]
% 	\end{tabular}}
%     \vspace{-2mm}
%     \caption{Performance of \algname under different vision token configurations on MiniCPM-V-2.6. In all experimental setups for \algname, the second layer is consistently designated as the pruned layer, with the total number of pivot tokens fixed at $8$. The pivot tokens are selected based on the maximum K-norm.}
%      \vspace{-2mm}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{4.0pt}
%     \renewcommand{\arraystretch}{1.3}
%     \footnotesize
% 	\centering
%     \begin{tabular}{p{2.5cm} | c c c c c c c | >{\centering\arraybackslash}p{1.2cm}}
%         \toprule[1.5pt]
%         \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.}\\
%         \hline
%         \rowcolor{mygray}
%         MiniCPM-V-2.6 & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$}   \\
%         \textcolor{gray}{Vanilla} & \textcolor{gray}{51.5} & \textcolor{gray}{79.7} & \textcolor{gray}{77.9} & \textcolor{gray}{2267} & \textcolor{gray}{83.2} & \textcolor{gray}{95.6} & \textcolor{gray}{78.5} & \multirow{1}*{\textcolor{gray}{100\%}} \\
%         \hline

%         \rowcolor{mygray}
%         MiniCPM-V-2.6 & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$}   \\
%         \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\%  \\
%         \hspace{0.5em} + \algname (Ours) & 47.8 & 76.5 & 74.8 & 1951 & 77.4 & 91.8 & 70.9 & 92.9\%  \\
%         \hline

%         \rowcolor{mygray}
%         MiniCPM-V-2.6 & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$}\\
%         \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\%  \\
%         \hspace{0.5em} + \algname (Ours) & 47.8 & 73.8 & 71.4 & 1821 & 71.6 & 88.9 & 65.7 & 88.6\%  \\
%         \hline

%         \rowcolor{mygray}
%         MiniCPM-V-2.6 & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$}\\
%         \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\%  \\
%         \hspace{0.5em} + \algname (Ours) & 42.5 & 66.2 & 64.0 & 1405 & 58.0 & 83.5 & 51.9 & 76.1\%  \\

%         \bottomrule[1.5pt]
% 	\end{tabular}
%         % \vspace{-2mm}
% 	\caption{Performance of \algname under different vision token configurations on MiniCPM-V-2.6. In all experimental setups for \algname, the second layer is consistently designated as the pruned layer, with the total number of pivot tokens fixed at $8$. The pivot tokens are selected based on the maximum K-norm.}
%     \label{tab:minicpm}
%      % \vspace{-2mm}
% \end{table*}

% -----------------------------
% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{4.0pt}
% \renewcommand{\arraystretch}{1.3}
% \footnotesize
% \begin{tabular}{p{2.5cm} | c c c c c c c | >{\centering\arraybackslash}p{1.2cm}}
% \toprule[1.5pt]
% \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.} \\
% \hline

% \rowcolor{mygray}
% \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$} \\
% \textcolor{gray}{Vanilla} & \textcolor{gray}{62.2} & \textcolor{gray}{80.5} & \textcolor{gray}{81.2} & \textcolor{gray}{2317} & \textcolor{gray}{86.1} & \textcolor{gray}{84.7} & \textcolor{gray}{82.1} & \textcolor{gray}{100\%} \\
% \hline

% \rowcolor{mygray}
% \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & 58.0 & 76.1 & 75.5 & 2130 & 82.1 & 80.0 & 77.3 & 94.0\% \\
% \hspace{0.5em} + \algname (Ours) & 60.2 & 78.9 & 78.0 & 2245 & 83.9 & 81.4 & 80.5 & 97.0\% \\
% \hline

% \rowcolor{mygray}
% \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & 56.7 & 74.1 & 73.9 & 2031 & 79.2 & 78.3 & 72.0 & 91.0\% \\
% \hspace{0.5em} + \algname (Ours) & 58.5 & 77.3 & 77.1 & 2175 & 82.1 & 79.6 & 75.3 & 94.3\% \\
% \hline

% \rowcolor{mygray}
% \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & 51.9 & 70.1 & 65.2 & 1962 & 76.1 & 75.8 & 60.3 & 84.0\% \\
% \hspace{0.5em} + \algname (Ours) & 55.5 & 72.0 & 71.7 & 2052 & 77.9 & 77.6 & 61.8 & 87.5\% \\
% \hline

% \rowcolor{cyan!20}
% \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$} \\
% \textcolor{gray}{Vanilla} & \textcolor{gray}{51.5} & \textcolor{gray}{79.7} & \textcolor{gray}{77.9} & \textcolor{gray}{2267} & \textcolor{gray}{83.2} & \textcolor{gray}{95.6} & \textcolor{gray}{78.5} & \textcolor{gray}{100\%} \\
% \hline

% \rowcolor{cyan!20}
% \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\% \\
% \hspace{0.5em} + \algname (Ours) & 47.8 & 76.5 & 74.8 & 1951 & 77.4 & 91.8 & 70.9 & 92.9\% \\
% \hline

% \rowcolor{cyan!20}
% \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\% \\
% \hspace{0.5em} + \algname (Ours) & 47.8 & 73.8 & 71.4 & 1821 & 71.6 & 88.9 & 65.7 & 88.6\% \\
% \hline

% \rowcolor{cyan!20}
% \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & - & - & - & - & - & - & - & -\% \\
% \hspace{0.5em} + \algname (Ours) & 42.5 & 66.2 & 64.0 & 1405 & 58.0 & 83.5 & 51.9 & 76.1\% \\
% \bottomrule[1.5pt]
% \end{tabular}
% \caption{Performance of \algname on Qwen2-VL-7B and MiniCPM-V-2.6 under different vision token configurations. For both models, the second layer is designated as the pruned layer with 8 fixed pivot tokens selected via maximum K-norm.}
% \label{tab:combined}
% \end{table*}



% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{4.0pt}
% \renewcommand{\arraystretch}{1.35}
% \footnotesize
% \begin{tabular}{p{2.5cm} c| c c c c c c c | >{\centering\arraybackslash}p{1.2cm}}
% \toprule[1.5pt]
% \textbf{Method} & \textbf{Reduction Ratio} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.} \\
% \hline

% % \rowcolor{mygray}
% % \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$} \\
% \textcolor{gray}{Qwen2-VL-7B} & \textcolor{gray}{$\downarrow 0.00\%$} & \textcolor{gray}{62.2} & \textcolor{gray}{80.5} & \textcolor{gray}{81.2} & \textcolor{gray}{2317} & \textcolor{gray}{86.1} & \textcolor{gray}{84.7} & \textcolor{gray}{82.1} & \textcolor{gray}{100\%} \\
% \hline

% % \rowcolor{mygray}
% % \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 66.7\%$ & 58.0 & 76.1 & 75.5 & 2130 & 82.1 & 80.0 & 77.3 & 94.0\% \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 66.7\%$ & 60.2 & 78.9 & 78.0 & 2245 & 83.9 & 81.4 & 80.5 & 97.0\% \\
% \hline

% % \rowcolor{mygray}
% % \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 77.8\%$ & 56.7 & 74.1 & 73.9 & 2031 & 79.2 & 78.3 & 72.0 & 91.0\% \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 77.8\%$ & 58.5 & 77.3 & 77.1 & 2175 & 82.1 & 79.6 & 75.3 & 94.3\% \\
% \hline

% % \rowcolor{mygray}
% % \textbf{Qwen2-VL-7B} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 88.9\%$ & 51.9 & 70.1 & 65.2 & 1962 & 76.1 & 75.8 & 60.3 & 84.0\% \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 88.9\%$ & 55.5 & 72.0 & 71.7 & 2052 & 77.9 & 77.6 & 61.8 & 87.5\% \\
% \hline
% \hline
% % \rowcolor{cyan!20}
% % \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$} \\
% \textcolor{gray}{MiniCPM-V-2.6} & - & \textcolor{gray}{51.5} & \textcolor{gray}{79.7} & \textcolor{gray}{77.9} & \textcolor{gray}{2267} & \textcolor{gray}{83.2} & \textcolor{gray}{95.6} & \textcolor{gray}{78.5} & \textcolor{gray}{100\%} \\
% \hline

% % \rowcolor{cyan!20}
% % \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 66.7\%$ & - & 74.9 & 73.1 & 1895 & 75.4 & 89.8 & 67.1 & -\%   \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 66.7\%$ & 47.8 & 76.5 & 74.8 & 1951 & 77.4 & 91.8 & 70.9 & 92.9\% \\
% \hline

% % \rowcolor{cyan!20}
% % \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 77.8\%$ & - & 72.9 & 70.4 & 1807 & - & 86.5 & 54.9 & -\% \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 77.8\%$ & 47.8 & 73.8 & 71.4 & 1821 & 71.6 & 88.9 & 65.7 & 88.6\% \\
% \hline

% % \rowcolor{cyan!20}
% % \textbf{MiniCPM-V-2.6} & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$} \\
% \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & $\downarrow 88.9\%$ & - & - & - & - & - & - & - & -\% \\
% \rowcolor{cyan!5}
% \hspace{0.5em} + \algname (Ours) & $\downarrow 88.9\%$ & 42.5 & 66.2 & 64.0 & 1405 & 58.0 & 83.5 & 51.9 & 76.1\% \\
% \bottomrule[1.5pt]
% \end{tabular}
% \caption{Comparative Experiments on Qwen2-VL-7B and MiniCPM-V-2.6 under different reduction ratio.}
% \label{tab:minicpm}
% \end{table*}





==> latex/content/table/image_understanding_qwen2vl.tex <==
% \renewcommand{\multirowsetup}{\centering}
% \definecolor{mygray}{gray}{.92}
% \definecolor{ForestGreen}{RGB}{34,139,34}
% \definecolor{Forestred}{RGB}{220,50,50}
% \begin{table*}[t]
%     \centering
%     % \hspace{2mm}
%     \scalebox{1.0}{
%     \setlength{\tabcolsep}{3.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \footnotesize
% 	\label{tab:qwen2vl}
%     \begin{tabular}{@{}lc | c c c c c c c | c}
%         \toprule[1.5pt]
%         \textbf{Method} & Retention Ratio & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} &  \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.} \\

%         \hline
%         Qwen2-VL-7B & $\fg{\downarrow 0.00\%}$ & \textcolor{gray}{62.2} & \textcolor{gray}{80.5} & \textcolor{gray}{81.2} & \textcolor{gray}{2317} & \textcolor{gray}{86.1} & \textcolor{gray}{84.7} & \textcolor{gray}{82.1} & \multirow{1}*{\textcolor{gray}{100\%}} \\

%         \hspace{0.5em} + \multirow{1}*{FastV \texttt{\scriptsize{(ECCV24)}}} & $\fg{\downarrow 66.7\%}$ & 58.0 & 76.1 & 75.5 & 2130 & 82.1 & 80.0 & 77.3 & -\% \\

%         \hspace{0.5em} + \multirow{1}*{FastV \texttt{\scriptsize{(ECCV24)}}} & $\fg{\downarrow 77.8\%}$ & - & - & - & - & - & - & - & -\% \\

%         \hspace{0.5em} + \multirow{1}*{FastV \texttt{\scriptsize{(ECCV24)}}} & $\fg{\downarrow 88.9\%}$ & - & - & - & - & - & - & - & -\%  \\

%         \hline

%         Qwen2-VL-7B & $\fg{\downarrow 0.00\%}$ & \textcolor{gray}{62.2} & \textcolor{gray}{80.5} & \textcolor{gray}{81.2} & \textcolor{gray}{2317} & \textcolor{gray}{86.1} & \textcolor{gray}{84.7} & \textcolor{gray}{82.1} & \multirow{1}*{\textcolor{gray}{100\%}} \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 66.7\%}$ & 60.2 & 78.9 & 78.0 & 2245 & 83.9 & 81.4 & 80.5 & 97.0\% \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 77.8\%}$ & 58.5 & 77.3 & 77.1 & 2175 & 82.1 & 79.6 & 75.3 & 94.3\% \\

%         \hspace{0.5em} + \multirow{1}*{\algname (Ours)} & $\fg{\downarrow 88.9\%}$ & 55.5 & 72.0 & 71.7 & 2052 & 77.9 & 77.6 & 61.8 & 87.5\%  \\
        

%         \bottomrule[1.5pt]
% 	\end{tabular}}
%         \vspace{-2mm}
%     \caption{Performance of \algname under different vision token configurations on Qwen2-VL-7B. In all experimental setups for \algname, the second layer is consistently designated as the pruned layer, with the total number of pivot tokens fixed at $8$. The pivot tokens are selected based on the maximum K-norm.}
%      \vspace{-2mm}
% \end{table*}



% \renewcommand{\multirowsetup}{\centering}
% \definecolor{mygray}{gray}{.92}
% \definecolor{ForestGreen}{RGB}{34,139,34}
% % \newcommand{\fg}[1]{\mathbf{\mathcolor{ForestGreen}{#1}}}
% \definecolor{Forestred}{RGB}{220,50,50}
% % \newcommand{\fr}[1]{\mathbf{\mathcolor{Forestred}{#1}}}
% \begin{table*}[t]
%     \centering
%     % \hspace{2mm}
%     \setlength{\tabcolsep}{4.0pt}
%     \renewcommand{\arraystretch}{1.3}
%     \footnotesize
% 	\centering
%     \begin{tabular}{p{2.5cm} | c c c c c c c | >{\centering\arraybackslash}p{1.2cm}}
%         \toprule[1.5pt]
%         \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB-CN} & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$^{\text{Text}}$ & \makecell[c]{\textbf{Avg}.}\\
%         \hline
%         \rowcolor{mygray}
%         Qwen2-VL-7B & \multicolumn{8}{c}{\textit{Upper Bound, All Tokens} \ $\textbf{(100\%)}$}   \\
%         \textcolor{gray}{Vanilla} & \textcolor{gray}{62.2} & \textcolor{gray}{80.5} & \textcolor{gray}{81.2} & \textcolor{gray}{2317} & \textcolor{gray}{86.1} & \textcolor{gray}{84.7} & \textcolor{gray}{82.1} & \multirow{1}*{\textcolor{gray}{100\%}} \\
%         \hline

%         \rowcolor{mygray}
%         Qwen2-VL-7B & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 66.7\%)}$}   \\
%         \hspace{0.5em} + FastV \texttt{\scriptsize{(ECCV24)}} & 58.0 & 76.1 & 75.5 & 2130 & 82.1 & 80.0 & 77.3 & 94.0\%  \\
%         \hspace{0.5em} + \algname (Ours) & 60.2 & 78.9 & 78.0 & 2245 & 83.9 & 81.4 & 80.5 & 97.0\%  \\
%         \hline

%         \rowcolor{mygray}
%         Qwen2-VL-7B & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 77.8\%)}$}\\
%         \hspace{0.5em} + \multirow{1}*{FastV \texttt{\scriptsize{(ECCV24)}}} & 56.7 & 74.1 & 73.9 & 2031 & 79.2 & 78.3 & 72.0 & 91.0\% \\
%         \hspace{0.5em} + \algname (Ours) & 58.5 & 77.3 & 77.1 & 2175 & 82.1 & 79.6 & 75.3 & 94.3\%  \\
%         \hline

%         \rowcolor{mygray}
%         Qwen2-VL-7B & \multicolumn{8}{c}{\textit{Token Reduction} \ $\fg{(\downarrow 88.9\%)}$}\\
%         \hspace{0.5em} + \multirow{1}*{FastV \texttt{\scriptsize{(ECCV24)}}} & 51.9 & 70.1 & 65.2 & 1962 & 76.1 & 75.8 & 60.3 & 84.0\%  \\
%         \hspace{0.5em} + \algname (Ours) & 55.5 & 72.0 & 71.7 & 2052 & 77.9 & 77.6 & 61.8 & 87.5\%  \\

%         \bottomrule[1.5pt]
% 	\end{tabular}
%         % \vspace{-2mm}
% 	\caption{Performance of \algname under different vision token configurations on Qwen2-VL-7B. In all experimental setups for \algname, the second layer is consistently designated as the pruned layer, with the total number of pivot tokens fixed at $8$. The pivot tokens are selected based on the maximum K-norm.}
%     \label{tab:qwen2vl}
%      % \vspace{-2mm}
% \end{table*}

==> latex/content/table/layer.tex <==
% \begin{table}[!t]
%     \centering
%     \caption{...}
%         \setlength{\tabcolsep}{1.0pt}
%             \renewcommand{\arraystretch}{1.2}
%             \footnotesize
%     \begin{tabular}{@{}lcccccc}
%         \toprule[1.2pt]
%          \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MME} & \textbf{SQA} & \textbf{VQA$^\text{V2}$} & \textbf{VQA$^\text{Text}$} \\
%          \hline
%          \rowcolor{mygray}
%          Vanilla & 61.9 & 64.7 & 1862 & 69.5 & 78.5 & 58.2 \\
%          \hline
%          \algname (K=1) & 58.6 & 63.7 & 1741 & 68.5 & 75.3 & 55.3 \\
%          \algname (K=2) & 58.7 & 63.2 & 1840 & 69.1 & 75.9 & 56.4 \\
%          \algname (K=3) & 59.5 & 63.9 & 1840 & 69.4 & - & 56.7 \\
       
%         \bottomrule[1.2pt]
%     \end{tabular}
%     \label{tab:layer}
% \end{table}


\begin{table}[!t]
    \centering
    \caption{retain 128 tokens.}
    \vspace{-2mm}
    \setlength{\tabcolsep}{2.5pt} % 调整列间距
    \renewcommand{\arraystretch}{1.0} % 增加行高
    \footnotesize % 缩小字体
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l|cccccc@{}}
        \toprule[1.2pt]
        \textbf{Method} & \textbf{GQA} & \textbf{MMB} & \textbf{MME} & \textbf{SQA} & \textbf{VQA$^\text{V2}$} & \textbf{VQA$^\text{Text}$} \\
        \midrule
        \textcolor{gray}{Vanilla} & \textcolor{gray}{61.9} & \textcolor{gray}{64.7} & \textcolor{gray}{1862} & \textcolor{gray}{69.5} & \textcolor{gray}{78.5} & \textcolor{gray}{58.2} \\
        \midrule
        & \multicolumn{6}{c}{\textbf{\textit{Retain 128 tokens}}} \\
        $K=1$ & 58.6 & 63.7 & 1741 & 68.5 & 75.3 & 55.3 \\
        $K=2$ & 58.7 & 63.2 & 1840 & 69.1 & 75.9 & 56.4 \\
        $K=3$ & 59.5 & 63.9 & 1840 & 69.4 & \multicolumn{1}{c}{-} & 56.7 \\
        $K=5$ & - & - & - & - & - & - \\
        $K=10$ & - & - & - & - & - & - \\
        \bottomrule[1.2pt]
    \end{tabular}%
    }
    \label{tab:layer}
    \vspace{-0.2cm} % 调整表格与下方内容的间距
\end{table}






==> latex/figure/radar_compare.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/radar_compare.pdf}
    % \vspace{-6mm}
    \caption{Comparison of LLaVA-1.5-7B on a range of 7 benchmarks, with a \textbf{88.9\%} reduction ratio. \algname outperforms other methods by a large margin on 6 tasks and achieves comparable results on the remaining one.}
    % \vspace{-4mm}
    \label{fig:radar_compare}
\end{figure}

==> latex/figure/radar_lalency.tex <==
% \begin{figure*}[t]
%   \centering
%   \begin{minipage}{0.35\linewidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figure/radar_compare.pdf}
%     \caption{...}
%     \label{fig:radar}
%   \end{minipage}
%   \hfill
%   \begin{minipage}{0.50\linewidth}
%     \centering
%     \includegraphics[width=1.05\linewidth, height=0.55\linewidth]{figure/latency_vs_performance.pdf}
%     \caption{...}
%     \label{fig:latency}
%   \end{minipage}
% %   \vspace{-5mm}
% \end{figure*}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/radar_latency_v2.pdf}
    % \vspace{-6mm}
    \caption{...}
    % \vspace{-4mm}
    \label{fig:radar_latency}
\end{figure*}
